An Educational System for Personalized Teacher Recommendation in K-12 Online Classrooms

In this paper, we propose a simple yet effective solution to build practical teacher recommender systems for online one-on-one classes. Our system consists of (1) a pseudo matching score module that provides reliable training labels; (2) a ranking model that scores every candidate teacher; (3) a novelty boosting module that gives additional opportunities to new teachers; and (4) a diversity metric that guardrails the recommended results to reduce the chance of collision. Offline experimental results show that our approach outperforms a wide range of baselines. Furthermore, we show that our approach is able to reduce the number of student-teacher matching attempts from 7.22 to 3.09 in a five-month observation on a third-party online education platform.

==> related.tex <==
In this section, we primarily focus on the recommendation systems. Collaborative filtering \cite{su2009survey,sarwar2001item}, matrix factorization \cite{koren2009matrix,rendle2010factorization} and content-based recommendation approaches \cite{lops2011content} are well studied and these approaches have become the foundations of recommender systems. A group of studies have been done to improve the existing performance. Tang, Hu, and Liu took time as an additional input dimension, aiming at explicitly modeling user interests over time \cite{tang2013social}.  Koren et al. developed a collaborative filtering type of approach with predictions from static average values combining with a dynamic changing factor \cite{koren2009collaborative}. Yin et al. proposed a user-tag-specific temporal interest model to track user interests over time by maximizing the time weighted data likelihood \cite{yin2011temporal}. For better personalization, Guy et al. proposed an item-based recommender system to utilize each user's social network information \cite{guy2009personalized}. A detailed review of recommender systems is out of the scope of this paper and please refer to \cite{bobadilla2013recommender,karimi2018news} for comprehensive summarizations. 

%\subsection{Teacher Recommendation}




